Code-Mixing on Sesame Street: Dawn of the Adversarial Polyglots

Multilingual models have demonstrated impressive cross-lingual transfer performance. However, test sets like XNLI are monolingual at the example level. In multilingual communities, it is common for polyglots to code-mix when conversing with each other. Inspired by this phenomenon, we present two strong black-box adversarial attacks (one word-level, one phrase-level) for multilingual models that push their ability to handle code-mixed sentences to the limit. The former uses bilingual dictionaries to propose perturbations and translations of the clean example for sense disambiguation. The latter directly aligns the clean example with its translations before extracting phrases as perturbations. Our phrase-level attack has a success rate of 89.75% against XLM-R-large, bringing its average accuracy of 79.85 down to 8.18 on XNLI. Finally, we propose an efficient adversarial training scheme that trains in the same number of steps as the original model and show that it improves model accuracy.

==> figs/cat_samples.tex <==
\begin{table}[h]
\small
    \centering
    \begin{tabular}{p{\linewidth}}
    \toprule
   \textbf{\poly\ Adversaries}\\
    \midrule
   Rockefeller {\greektext έδωσε} to \AR{السرطان} forschung.\\
   \midrule
   	The \begin{CJK*}{UTF8}{gbsn}发音 列表\end{CJK*} \foreignlanguage{russian}{само} included the most basic things.\\
    \midrule
    He vardı yedi hermanas and no brothers in his family.\\
    \midrule
    But même {\greektext хотя} as a boy I lived on a çiftlik right on the Mexican \AR{حدود}, I \AR{تذكر} being mystified by ranching términos that crept into Western songs du north of us, cayuse, for example.\\
    \midrule
	We should nie think of human equality when we consider social and political justice.\\
    \bottomrule
    \end{tabular}
    \caption{\poly\ adversaries for XLM-R$_\text{base}$ on XNLI-13.}
    \label{tab:poly_adv}
\end{table}

\begin{table}[h]
\small
    \centering
    \begin{tabular}{p{\linewidth}}
    \toprule
   \textbf{Code-Mixed Adversarial Training Examples}\\
    \midrule
    Not much has sich innerhalb des Jahrzehnts verändert.\\
    \midrule
    Ese \AR{كان} el most historic weather \AR{يوم} in la historia registrada para el el clima severo en el country \\
    \midrule
    Como ustedes {\greektext γνωρίζετε}, last enero hemos issued un {\greektext νέο όγκο} de reports, la Performance {\greektext και λογοδοσίας} serie de, en los que se esbozan los de gestión desafíos {\greektext που αντιμετωπίζουν οι} nuestras mayores federal agencies and the substantial opportunities para mejorar su rendimiento.\\
    \midrule
    because a lot \foreignlanguage{vietnamese}{trong số họ} are are similar	\\
    \midrule
    um-hum bueno that's increíble como i used to cuando i was \foreignlanguage{russian}{в} college solía la have el stereo en all \foreignlanguage{russian}{през} time or i tenía en MTV or something but ever que i've been out de college
    \bottomrule
    \end{tabular}
    \caption{Code-mixed adversarial training examples.}
    \label{tab:cat_samples}
\end{table}
